Transparent Checkpointing for OpenGL Applications on GPUs

This work presents transparent checkpointing of OpenGL applications, refining the split-process technique[1] for application in GPU-based 3D graphics. The split-process technique was earlier applied to checkpointing MPI and CUDA programs, enabling reinitialization of driver libraries. The presented design targets practical, checkpoint-package agnostic checkpointing of OpenGL applications. An early prototype is demonstrated on Autodesk Maya. Maya is a complex proprietary media-creation software suite used with large-scale rendering hardware for CGI (Computer-Generated Animation). Transparent checkpointing of Maya provides critically-needed fault tolerance, since Maya is prone to crash when artists use some of its bleeding-edge components. Artists then lose hours of work in re-creating their complex environment.

==> Makefile <==
FILE=ckpt-opengl

pdf: ${FILE}.tex ${FILE}.bib
	pdflatex $<
	bibtex ${FILE}

okular: ${FILE}.pdf
	okular $<

vi vim touch: ${FILE}.tex
	$@ $<

spell: ${FILE}.tex detex.sed
	cat $< | sed -f detex.sed | spell | sort | uniq

dist: clean
	dir=`basename $$PWD` && cd .. && \
	  tar zcvf $$dir.tgz --exclude=$$dir/.git $$dir
	dir=`basename $$PWD` && ls -l ../$$dir.tgz

clean:
	for type in aux bbl blg log out; do \
	  rm -f ${FILE}.$$type; \
	done

